GLaMM: Pixel Grounding Large Multimodal Model

Large Multimodal Models (LMMs) extend Large Language Models to the vision domain. Initial LMMs used holistic images and text prompts to generate ungrounded textual responses. Recently, region-level LMMs have been used to generate visually grounded responses. However, they are limited to only referring to a single object category at a time, require users to specify the regions, or cannot offer dense pixel-wise object grounding. In this work, we present Grounding LMM (GLaMM), the first model that can generate natural language responses seamlessly intertwined with corresponding object segmentation masks. GLaMM not only grounds objects appearing in the conversations but is flexible enough to accept both textual and optional visual prompts (region of interest) as input. This empowers users to interact with the model at various levels of granularity, both in textual and visual domains. Due to the lack of standard benchmarks for the novel setting of visually Grounded Conversation Generation (GCG), we introduce a comprehensive evaluation protocol with our curated grounded conversations. Our proposed GCG task requires densely grounded concepts in natural scenes at a large-scale. To this end, we propose a densely annotated Grounding-anything Dataset (GranD) using our proposed automated annotation pipeline that encompasses 7.5M unique concepts grounded in a total of 810M regions available with segmentation masks. Besides GCG, GLaMM also performs effectively on several downstream tasks, e.g., referring expression segmentation, image and region-level captioning and vision-language conversations.

==> main_cvpr.tex <==
% % CVPR 2024 Paper Template; see https://github.com/cvpr-org/author-kit

% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE  - PLEASE UPDATE FOR FINAL VERSION
% \usepackage{cvpr}              % To produce the CAMERA-READY version
% % \usepackage[review]{cvpr}      % To produce the REVIEW version
% % \usepackage[pagenumbers]{cvpr} % To force page numbers, e.g. for an arXiv version

% % Import additional packages in the preamble file, before hyperref
% \input{preamble}

% % It is strongly recommended to use hyperref, especially for the review version.
% % hyperref with option pagebackref eases the reviewers' job.
% % Please disable hyperref *only* if you encounter grave issues, 
% % e.g. with the file validation for the camera-ready version.
% %
% % If you comment hyperref and then uncomment it, you should delete *.aux before re-running LaTeX.
% % (Or just hit 'q' on the first LaTeX run, let it finish, and you should be clear).
% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
% \usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}
% %-- Additional packages-----%
% \usepackage{inconsolata}
% \usepackage{multirow}
% \usepackage{tabularx}
% \usepackage{colortbl}
% \usepackage{pifont}
% \usepackage{multicol}
% \usepackage{xcolor}
% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\paperID{*****} % *** Enter the Paper ID here
% \def\confName{CVPR}
% \def\confYear{2024}

% \usepackage{colortbl}
% \usepackage{xcolor}
% \definecolor{tabhighlight}{HTML}{e5e5e5}
% %-- Additional Commands-----%
% \renewcommand{\ttdefault}{zi4}
% \definecolor{mydarkgreen}{rgb}{0.0, 0.5, 0.0}  % Adjust the RGB values to your preference
% \newcommand{\cmark}{\textcolor{mydarkgreen}{\scalebox{1}[1.0]{\ding{51}}}}
% \newcommand{\xmark}{\textcolor{red}{\ding{55}}}  % Cross
% % --------
% \usepackage{color}
% \usepackage{marvosym}
% \usepackage{enumitem}
% \usepackage{utfsym}
% \usepackage{xspace}
% \usepackage{pifont}
% \usepackage[T1]{fontenc}
% \definecolor{citecolor}{HTML}{0071BC}
% \definecolor{linkcolor}{HTML}{ED1C24}

% \newcommand{\sfc}[1]{\textcolor{blue}{#1}}
% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{GLaMM \includegraphics[width=0.04\linewidth]{Figures/GlamImage-min.png}: Grounding Large Multimodal Model}
% % \title{MaRVEL: Any-to-Any Large Vision Language Model for Visual Grounding and Understanding}
% % \title{MaRVEL: Any-to-Any Large Vision Language Model for Multimodal Grounding and Understanding}
% %%%%%%%%% AUTHORS - PLEASE UPDATE
% % \author{First Author\\
% % Institution1\\
% % Institution1 address\\
% % {\tt\small firstauthor@i1.org}
% % % For a paper whose authors are all at the same institution,
% % % omit the following lines up until the closing ``}''.
% % % Additional authors and addresses can be added with ``\and'',
% % % just like the second author.
% % % To save space, use either the email address or home page, not both
% % \and
% % Second Author\\
% % Institution2\\
% % First line of institution2 address\\
% % {\tt\small secondauthor@i2.org}
% % }
% % \author{%
% %   Hanoona Rasheed\textsuperscript{\textnormal{*}}, Muhammad Maaz\textsuperscript{\textnormal{*}} \\
% %   Sahal Shaji, Abdelrahman Shaker, Salman Khan\\
% %   Hisham Cholakkal, Rao Muhammad Anwer, Fahad Shahbaz Khan\\
% %   \texttt{hanoona.bangalath@mbzuai.ac.ae, muhammad.maaz@mbzuai.ac.ae}\\
% %   Mohamed bin Zayed University of AI  \\
% % %   \texttt{\{first\_name\}.\{surname\}@unibe.ch} \\
% % }
% \author{%
%   Hanoona Rasheed\textsuperscript{\textnormal{*}}, Muhammad Maaz\textsuperscript{\textnormal{*}} Sahal Shaji, Abdelrahman Shaker\\
%   Salman Khan, Hisham Cholakkal, Rao Muhammad Anwer, Fahad Shahbaz Khan\\
%   \texttt{hanoona.bangalath@mbzuai.ac.ae, muhammad.maaz@mbzuai.ac.ae}\\
%   Mohamed bin Zayed University of AI  \\
% %   \texttt{\{first\_name\}.\{surname\}@unibe.ch} \\
% }

% \begin{document}
% \maketitle
% \input{sec/0_abstract}    
% \input{sec/1_intro}
% \input{sec/2_related}
% \input{sec/4_method}
% \input{sec/3_dataset}
% \input{sec/5_experiments}
% \input{sec/conclusion}
% {
%     \small
%     \bibliographystyle{ieeenat_fullname}
%     \bibliography{main}
% }
% \input{sec/X_suppl}
% % WARNING: do not forget to delete the supplementary pages from your submission 
% % \input{sec/X_suppl}

% \end{document}

